Optically Loaded Semiconductor Quantum Memory Register

We propose and analyze an optically loaded quantum memory exploiting capacitive coupling between self-assembled quantum dot molecules and electrically gated quantum dot molecules. The self-assembled dots are used for spin-photon entanglement, which is transferred to the gated dots for long-term storage or processing via a teleportation process heralded by single-photon detection. We illustrate a device architecture enabling this interaction and we outline its operation and fabrication. We provide self-consistent Poisson-Schroedinger simulations to establish the design viability and refine the design, and to estimate the physical coupling parameters and their sensitivities to dot placement. The device we propose generates heralded copies of an entangled state between a photonic qubit and a solid-state qubit with a rapid reset time upon failure. The resulting fast rate of entanglement generation is of high utility for heralded quantum networking scenarios involving lossy optical channels.

==> device_design_header.tex <==
\RequirePackage{varioref}
\RequirePackage{amsmath}
\RequirePackage{amssymb}
\RequirePackage{bm}
\RequirePackage{graphicx}
\RequirePackage{color}
\RequirePackage[active]{srcltx}
%\RequirePackage{draftwatermark}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Long comments
\long\def\comment#1{}

%%%%%%%%%%%%%%%%%%%%%%%%%%%% To save typing on all math commands
\newcommand{\mathcommand}[3][0]{\newcommand{#2}[#1]{\ensuremath{#3}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Text subscripting
\newcommand{\ts}[2]{{#1}_{\textnormal{#2}}} %A math symbol with a text subscript
\newcommand{\tsc}[2]{{#1}_{\textsc{\lowercase{#2}}}} %A math symbol with a text subscript, small caps

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Abbreviations
\newcommand{\abbrev}[1]{{\scshape\lowercase{#1}}}  % see LaTeX Companion, p. 169

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% More commands
%%%%%%%%%%%%%%%%%%%%%%%%%%%% Referencing Equations
% Uses package varioref
\renewcommand{\reftextcurrent}{}
\newcommand{\refeq}[1]{Eq.~\eqref{#1}}
\newcommand{\refequation}[1]{Equation~\eqref{#1}}
\newcommand{\fullrefeq}[1]{Eq.~\eqref{#1} \vpageref{#1}}
\newcommand{\fullrefequation}[1]{Equation~\eqref{#1} \vpageref{#1}}
\newcommand{\reftwoeqs}[2]{Eqs.~\eqref{#1} and \eqref{#2}}
\newcommand{\refeqs}[1]{Eqs.~\eqref{#1}}
\newcommand{\refsec}[1]{Sec.~\ref{#1}}
\newcommand{\refexteq}[1]{Eq.~(#1)}
\newcommand{\reftable}[1]{Table~\ref{#1}}
\newcommand{\reffig}[1]{Fig.~\ref{#1}}
\newcommand{\refchapter}[1]{Chapter~\ref{#1}}
\newcommand{\refapp}[1]{Appendix~\ref{#1}}
\newcommand{\ibid}{\latinfont{ibid}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%% Hamiltonian Notation
\newcommand{\ham}[1][]{\ensuremath{{H}_{\text{#1}}}} % symbol for hamiltonian (second quantized)
\newcommand{\tildeham}[1][]{\ensuremath{{\tilde{H}}_{\text{#1}}}}
\newcommand{\hamdens}[1][]{\ensuremath{\mathcal{H}_{\text{#1}}}} %symbol for hamiltonian density
\newcommand{\tildehamdens}[1][]{\ensuremath{\tilde{\mathcal{H}}_{\text{#1}}}} %symbol for hamiltonian density with tilde
\newcommand{\barhamdens}[1][]{\ensuremath{\ts{\bar{\mathcal{H}}}{#1}}}
\mathcommand[1]{\supop}{\hat{#1}} % to promote an operator to a superoperator
\newcommand{\supham}[1][]{\ensuremath{\supop{H}_{\text{#1}}}} %symbol for hamiltonian superoperator
\mathcommand[1]{\hilbert}{\mathfrak{H}_{\text{#1}}} %symbol for Hilbert space
\newcommand{\aveham}[2][]{\bar{\mathcal{H}}^{(#2)}_{\text{#1}}} % Used for average Hamiltonian terms in paper
\mathcommand[2]{\avehamt}{\ts{\tilde{\mathcal{H}}}{#1}^{(#2)}} % Used for average Hamiltonian terms in paper
\mathcommand\hc{\text{~h.c.}}

\mathcommand{\DOS}{\mathcal{D}}  % density of states

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Bra Ket notation
\mathcommand[1]{\smallket}{|#1\rangle}
\mathcommand[1]{\smallbra}{\langle #1|}
\mathcommand[1]{\bigket}{\bigl|#1\bigr\rangle}
\mathcommand[1]{\bigbra}{\bigl\langle #1\bigr|}
\mathcommand[1]{\biggket}{\biggl|#1\biggr\rangle}
\mathcommand[1]{\biggbra}{\biggl\langle #1\biggr|}
\mathcommand[1]{\ket}{\left| #1 \right\rangle}  %a Ket
\mathcommand[1]{\lket}{\bigl| #1 \bigr)}  %a Liouville Ket
\mathcommand[1]{\bra}{\left\langle #1 \right|}  %a Bra
\mathcommand[1]{\lbra}{\bigl( #1 \bigr|}  %a Bra
\newcommand{\ketbra}[2]{\left| #1 \right\rangle\!\!\left\langle #2
\right|} %an outer product
\newcommand{\braket}[2]{\left\langle #1 |#2\right\rangle} %an inner product
\newcommand{\bigbraket}[2]{\bigl\langle #1 \bigl| #2 \bigr\rangle} %an inner product
\newcommand{\biggbraket}[2]{\biggl\langle #1 \biggl| #2 \biggr\rangle} %an inner product
\newcommand{\bigketbra}[2]{\bigl| #1 \bigr\rangle\!\bigl\langle #2
\bigr|} %an outer product
\newcommand{\lbraket}[2]{\bigl( #1 \bigl| #2 \bigr)} %an inner product
\newcommand{\lketbra}[2]{\bigl| #1 \bigr)\!\!\bigl( #2
\bigr|} %an outer product
\newcommand{\sizedlbraket}[2]{\left.\left( #1 \left| #2 \right)\right.\right.} %an inner product
\newcommand{\biglbraket}[2]{\biggl(#1\biggl|#2\biggr)}
    % This one (above) scales to the right size, but:
    % works only if bra is smaller than ket
    % If something else is needed, define \rbraket
    % These Always make big delimiters
\newcommand{\bbraket}[2]{\biggl\langle #1 \biggm| #2 \biggr\rangle}
\mathcommand[1]{\bbra}{\biggl\langle #1 \biggr|}
\mathcommand[1]{\bket}{\biggl| #1 \biggr\rangle}
\newcommand{\gsket}{\ket{\Omega}}  %Ground state
\newcommand{\gsbra}{\bra{\Omega}}

\mathcommand{\upket}{\ket{\uparrow}}
\mathcommand{\downket}{\ket{\downarrow}}
\mathcommand{\upbra}{\bra{\uparrow}}
\mathcommand{\downbra}{\bra{\downarrow}}
\mathcommand{\upupket}{\ket{\uparrow\uparrow}}
\mathcommand{\updownket}{\ket{\uparrow\downarrow}}
\mathcommand{\downupket}{\ket{\downarrow\uparrow}}
\mathcommand{\downdownket}{\ket{\downarrow\downarrow}}

\mathcommand{\cnot}{\text{c-}\textsc{not}}
\mathcommand{\cZ}{\text{c-}Z}

%%%%%%%%%%%%%%%%%%%%%%%%% Phantom commands
\newcommand{\nodag}{{\phantom{\dag}}} %use c^\nodag to space it like c^\dag
\newcommand{\nostar}{{\phantom{*}}} % not sure if this will work

%%%%%%%%%%%%%%%%%%%%%%%%%%%% Trace
\newcommand{\Tr}[2][]{\text{Tr}_\text{#1}\left\{#2\right\}}

%%%%%%%%%%%%%%%%% Some common vectors
\renewcommand{\vec}[1]{\ensuremath{\text{\textbf{#1}}}} % Simply a bold charactor.
    % Boldsymbol in addition to \mathbf works for Greek letters

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Equation Environments
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\splitstart}{\begin{equation}\begin{split}}
\newcommand{\splitstop}{\end{split}\end{equation}} %Why doesn't this work?!?

%%%%%%%%%%%%%%%%%%% Miscellaneous
\mathcommand{\infinity}{\infty}
\renewcommand{\Im}[1]{\ensuremath{
    \text{Im}\left\{#1\right\}}}
\renewcommand{\Re}[1]{\ensuremath{
    \text{Re}\left\{#1\right\}}}
\mathcommand{\dftnorm}{\frac{1}{\sqrt{N}}}
\mathcommand{\onehalf}{\frac{1}{2}}
\mathcommand[1]{\nth}{#1^{\text{th}}}
\mathcommand[4]{\columnvector}{\left(\begin{array}{c}
            #1\\#2\\#3\\#4 \end{array}\right)}
\mathcommand[4]{\specfunc}{#1_{#2}^{#3}\!\!\left(#4\right)} %For example, spherical harmonic, Laguerre polynomials
\newcommand{\partialby}[1]{\frac{\partial}{\partial{#1}}}
\newcommand{\sqpartialby}[1]{\frac{\partial^2}{\partial{#1}^2}}
\newcommand{\dbyd}[1]{\frac{d}{d#1}}
\mathcommand{\radtwo}{\sqrt{2}}
\mathcommand[1]{\oneover}{\frac{1}{#1}}
\newcommand{\mymatrix}[1]{\left(\begin{array}{ccc} #1
\end{array}\right)}
\newcommand{\rmatrix}[1]{\left(\begin{array}{rrr} #1
\end{array}\right)}
\mathcommand[1]{\specialsum}{{\sum_{#1}}^*}

%%%%%%%%%%%%%%%%%%%%% functions
\mathcommand{\erf}{{\rm erf}}
\mathcommand{\erfc}{{\rm erfc}}
\mathcommand{\sech}{{\rm sech}}
\mathcommand{\csch}{{\rm csch}}
\newcommand{\sinc}[1][]{\ensuremath{{\rm sinc}_{#1}}}
\mathcommand[1]{\floor}{\left\lfloor #1 \right\rfloor}
\mathcommand[1]{\ceil}{\left\lceil #1 \right\rceil}

%%%%%%%%%%%%%%%%%%% Struts
\newcommand{\mystrut}{\rule{0pt}{2.3ex}} % An x is the height of the LC letter x
\newcommand{\tablestrut}{\rule{0ex}{2.6ex}} % Gratzer, p. 151

%%%%%%%%%%%%%%%%%%% See p. 108, LaTeX Companion
\newcommand{\PBS}[1]{\let\temp=\\ #1 \let\\=\temp}
\newcommand{\narrowcol}{\PBS\raggedright\hspace{0pt}}

%%%%%%%%%%%%%%%%%%%%%%% Latin
\newcommand{\latinfont}[1]{#1}  % I think this is what the Chi. Man. of Style suggests
%\newcommand{\latinfont}[1]{\textit{#1}}
\newcommand{\ie}{\latinfont{i.e.}}
\newcommand{\via}{\latinfont{via}}
\newcommand{\eg}{\latinfont{e.g.}}
\newcommand{\cf}{\latinfont{cf.}}
\newcommand{\etal}{\latinfont{et al.}} %Note period is omitted to be used in BibTeX
\newcommand{\vs}{\latinfont{vs.}}
% I don't know how to change the et al. used by BibTeX, and it is not italic.
% kluge solution:
\newcommand{\bibetal}[2]{{#1 #2 \etal}}

%%%%%%%%%%%%%%%%%%%%%%% Temp fig
\newcommand{\tempfig}[4]{
    \begin{figure}
    \centering
    \boxed{
    \makebox[#1][c]{
    \begin{tabular}{c}
    \rule{0pt}{#2} \\
    \Huge #3 \\
    \rule{0pt}{#2}\\
    \end{tabular}}}
    \caption{#4 \label{#3}}
    \end{figure}}

% Some common colors
\newcommand{\green}{\textcolor[rgb]{0,0.4,0}}
\newcommand{\purple}{\textcolor[rgb]{0.8,0.2,0.6}} %Chosen to match standard Powerpoint colors
\newcommand{\blue}{\textcolor[rgb]{0,0,0.7}}
\newcommand{\red}{\textcolor{red}}
\newcommand{\teal}{\textcolor[rgb]{0,0.4,0.3}}
\newcommand{\darkyellow}{\textcolor[rgb]{0.8,0.6,0}}
\newcommand{\orange}{\textcolor[rgb]{1,0.4,0}}

% dense lists
\newenvironment{denseitemize}
    {\begin{list}{$\bullet$}{%
        \setlength{\topsep}{0in}
        \setlength{\parsep}{0in}
        \setlength{\itemsep}{0in}
        \setlength{\labelwidth}{3ex}
        \setlength{\leftmargin}{\labelwidth}
        \setlength{\rightmargin}{0in}
        }%
    }%
{\end{list}}

\newenvironment{densesubitemize}
    {\begin{list}{$-$}{%
        \setlength{\topsep}{0in}
        \setlength{\parsep}{0in}
        \setlength{\itemsep}{0in}
        \setlength{\rightmargin}{0in}
        }%
    }%
{\end{list}}

\newcounter{denseenumeratecounter}
\newlength{\denseenumeratelabel}
\settowidth{\denseenumeratelabel}{99.\hfil}
\newenvironment{denseenumerate}
    {\setcounter{denseenumeratecounter}{0}
        \begin{list}{\arabic{enumi}}{%
        \setlength{\topsep}{0in}
        \setlength{\parsep}{0in}
        \setlength{\itemsep}{0in}
        \setlength{\labelwidth}{\denseenumeratelabel}
        \setlength{\leftmargin}{\labelwidth}
        \addtolength{\leftmargin}{3pt}
        \setlength{\rightmargin}{0in}
        \renewcommand{\makelabel}[1]{%
            \stepcounter{denseenumeratecounter}
            \arabic{denseenumeratecounter}.\hfil}
        }%
    }%
{\end{list}}
\newcommand\Ci{\text{Ci}}
\mathcommand{\ta}{\boldsymbol\tau}
\mathcommand{\ev}{\boldsymbol\epsilon}
\mathcommand[1]{\cvec}{\overline{#1}}
\mathcommand{\trmat}{\cvec{\text{Tr}}}

\newcommand{\tc}[1]{\red{$\rightarrow$#1$\leftarrow$}\\} % temporary comment

\mathcommand\tO{\ts{t}{O}}
\mathcommand\tE{\ts{t}{E}}
\mathcommand{\Sket}{\ts{\ket{S}}{O}}
\newcommand{\Optical}[1]{\ts{#1}{O}}
\mathcommand{\Tket}{\Optical{\ket{T_0}}}
\mathcommand{\Tbra}{\bra{T_0}}
\mathcommand\JO{\Optical{J}}
\mathcommand\JE{\ts{J}{E}}
\mathcommand\JOE{\ts{J}{OE}}
\mathcommand\vac{\ket{\text{vac}}}
\mathcommand\tCZ{\ts{t}{CZ}} 
